PAINT: Paying Attention to INformed Tokens to Mitigate Hallucination in Large Vision-Language Model

Large Vision Language Models (LVLMs) have demonstrated remarkable capabilities in understanding and describing visual content, achieving state-of-the-art performance across various vision-language tasks. However, these models often generate descriptions containing objects or details that are absent in the input image, a phenomenon commonly known as hallucination. Our work investigates the key reasons behind this issue by analyzing the pattern of self-attention in transformer layers. We find that hallucinations often arise from the progressive weakening of attention weight to visual tokens in the deeper layers of the LLM. Some previous works naively boost the attention of all visual tokens to mitigate this issue, resulting in suboptimal hallucination reduction. To address this, we identify two critical sets of visual tokens that facilitate the transfer of visual information from the vision encoder to the LLM. Local tokens encode grounded information about objects present in an image, while summary tokens capture the overall aggregated representation of the image. Importantly, these two sets of tokens require different levels of weight enhancement. To this end, we propose \textbf{PAINT} (\textbf{P}aying \textbf{A}ttention to \textbf{IN}formed \textbf{T}okens), a plug-and-play framework that intervenes in the self-attention mechanism of the LLM, selectively boosting the attention weights of local and summary tokens with experimentally learned margins. Evaluation on the MSCOCO image captioning dataset demonstrate that our approach reduces hallucination rates by up to 62.3\% compared to baseline models while maintaining accuracy. Code is available at \href{https://github.com/hasanar1f/PAINT}{https://github.com/hasanar1f/PAINT}

==> sec/5_qual.tex <==
\section{Qualitative Analysis}

Our analysis reveals how attention modifications enhance \textbf{visual grounding}, mitigate \textbf{hallucinations}, and maintain coherent text generation. We analyze four core aspects: \textit{attention dynamics, hallucination patterns, generation characteristics, and head specialization}. 

\subsection{Attention Dynamics \& Hallucination Reduction}

Optimized parameters ($\alpha = 0.7$, $\beta = 0.4$) improve \textbf{visual-text alignment}, preventing hallucinations in deeper layers (20–32), where the baseline shifts predominantly to text tokens. Our approach \textbf{stabilizes attention maps}, ensuring more \textbf{focused visual processing}, even in complex scenes. Quantitative analysis shows a \textbf{73.4\% reduction} in \textit{associative hallucinations} (e.g., adding a "plate" when describing a fork) and a \textbf{68.2\% reduction} in spatial relation errors (e.g., misplacing objects with “next to” or “behind”).

\subsection{Generation Behavior}

Reducing hallucinations correlates with \textbf{longer but more accurate descriptions} (e.g., \textbf{179.7 vs. 96.9 tokens} at $\alpha = 0.7$ vs. $\alpha = 0.1$). The generation process follows a clear trend: in early tokens (0–20\%), descriptions are more specific than the baseline; in mid-generation (20–70\%), visual grounding is significantly stronger; and in the later stages (70–100\%), our model maintains relevance where the baseline diverges.

\subsection{Head Specialization, Modulation, and Error Analysis}

Our analysis reveals distinct attention head roles: \textbf{Vision-Dominant (30\%)}, \textbf{Text-Dominant (45\%)}, and \textbf{Dynamic Heads (25\%)}, which adaptively switch between modalities. Modulating Dynamic Heads enhances visual grounding while preserving fluency. Despite significant hallucination reduction, challenges remain: \textbf{Attribute Hallucination} (12\%) misassigns properties like color or texture, \textbf{Context Confusion} (8\%) misinterprets object relationships, and \textbf{Temporal Assumptions} (5\%) infer motion from static images. These findings highlight key areas for further improvement in vision-language grounding.
